LLM-Agents Driven Automated Simulation Testing and Analysis of small Uncrewed Aerial Systems

Thorough simulation testing is crucial for validating the correct behavior of small Uncrewed Aerial Systems (sUAS) across multiple scenarios, including adverse weather conditions (such as wind, and fog), diverse settings (hilly terrain, or urban areas), and varying mission profiles (surveillance, tracking). While various sUAS simulation tools exist to support developers, the entire process of creating, executing, and analyzing simulation tests remains a largely manual and cumbersome task. Developers must identify test scenarios, set up the simulation environment, integrate the System under Test (SuT) with simulation tools, formulate mission plans, and collect and analyze results. These labor-intensive tasks limit the ability of developers to conduct exhaustive testing across a wide range of scenarios. To alleviate this problem, in this paper, we propose AutoSimTest, a Large Language Model (LLM)-driven framework, where multiple LLM agents collaborate to support the sUAS simulation testing process. This includes: (1) creating test scenarios that subject the SuT to unique environmental contexts; (2) preparing the simulation environment as per the test scenario; (3) generating diverse sUAS missions for the SuT to execute; and (4) analyzing simulation results and providing an interactive analytics interface. Further, the design of the framework is flexible for creating and testing scenarios for a variety of sUAS use cases, simulation tools, and SuT input requirements. We evaluated our approach by (a) conducting simulation testing of PX4 and ArduPilot flight-controller-based SuTs, (b) analyzing the performance of each agent, and (c) gathering feedback from sUAS developers. Our findings indicate that AutoSimTest significantly improves the efficiency and scope of the sUAS testing process, allowing for more comprehensive and varied scenario evaluations while reducing the manual effort.

==> tables/a-agent-knowledge-base.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{|c|p{3cm}|c|c|}
\hline
\textbf{No.} & \textbf{Source Type} & \textbf{Parameter Count} & \textbf{Tokens} \\
\hline
1 & Source Code \cite{} &  & \\
\hline
2 & Documentation \cite{} &  & \\
\hline

\end{tabular}
    \caption{Data Sources to build \aagent Knowledge Base}
    \label{table:s-agent-knowledge-base}
\end{table}



==> tables/backup-from-table.tex <==
\begin{table*}[h]

\centering
\renewcommand{\arraystretch}{1.22}
\begin{tabularx}
{\textwidth}{|m{0.04\textwidth}|m{0.19\textwidth}|m{0.18\textwidth}|m{0.17\textwidth}|m{0.18\textwidth}|m{0.10\textwidth}|}
\hline
\textbf{Prompt} & \textbf{S-Agent} & \textbf{M-Agent} & \textbf{Env-Agent} & \textbf{A-Agent (Automated)} & \textbf{A-Agent (Interactive)} \\ \hline \textbf{Agent Goals} & generate  scenario blueprints that include 
\begin{itemize}[leftmargin=*]
    \item[-] Environment
    \item[-]Mission
    \item[-] Test Props
\end{itemize} & generate a SuT mission script based on scenario blueprint & generate sim tool script based on scenario blueprint &  Analyze simulation log data and explain how the test properties are affected & NA \\ \hline
\textbf{User Goals} &\textit{Example}: Generate a search-and-rescue mission scenarios  & NA & NA & NA & \textit{Example}: Explain all px4 parameters that might have an impact of high wind \\ \hline
\textbf{Sample} & Ref Example blueprint in Section \ref{subsec:phase1} & Ref Figure \ref{fig:magent} & Ref Figure \ref{fig:eagent} & NA & NA \\ \hline
\textbf{Rules} & 
\begin{itemize}
    % \item Output not equals Sample
    \item Blueprint Completeness
    
\end{itemize}
% (i) the generated scenario blueprints must include all higher level details described in the Agent's Goals, and (ii) that the agent should not directly copy anything from the sample of scenario provided to generate the response
& 
\begin{itemize}
    \item Script Format Validity
    \item Valid Geo-loc 
    \item Valid Waypoints 
    \item Velocity = [0,30] mph
    \item Altitude \leq 400 ft
   
\end{itemize}
% Ensure that the geolocations are valid and in close proximity. Ensure that mission waypoint contains values for 3D coordinate system.  Ensure that velocity is with-in 3 - 30 mph range. Ensure that Altitude information is always below 400 feet.  

& 
\begin{itemize}
    \item Script Format Validity
    \item Wind = [0,50] mph
    \item Light Intensity=(0,10)
    
\end{itemize}

% Ensure that the generated script is valid and adheres to the format of expected sample output. Ensure that the time of day is not night. Ensure that wind values are not above 50 mph. 
& 
\begin{itemize}
    \item Analysis Completeness 
\end{itemize}

% (a) ensure that analysis is conducted for all higher order metrics described in the Agent's Goals, and (b) verify that the complete simulation log metadata is considered to generate the analysis to avoid any gaps in the analysis. 

& NA  \\ \hline
\textbf{Data} &  List of past sUAS incidents in the real world & NA & NA & NA & Flight Controller Codebase and Documentation \\ \hline
\end{tabularx}
\label{tab:prompt-design}
\caption{Prompt Design}
\end{table*}




==> tables/s-agent-qual.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Use-Case & Scenario ID & Environment & Weather & Time of Day & Mission Complexity \\
\hline
Search and Rescue & 1-5 & Forest (3), Urban (1), Rural (1) & Rainy (2), Clear (2), Windy (1) & Day (3), Night (2) & Moderate (4), Complex (1) \\
\hline
Surveillance & 6-10 & Urban (4), Rural (1) & Clear (4), Cloudy (1) & Night (4), Day (1) & Simple (3), Moderate (2) \\
\hline
Inspection & 11-15 & Rural (3), Forest (2) & Windy (2), Clear (2), Rainy (1) & Dawn (2), Day (3) & Complex (4), Moderate (1) \\
\hline
Package Delivery & 16-20 & Urban (4), Rural (1) & Clear (4), Rainy (1) & Day (4), Night (1) & Simple (4), Moderate (1) \\
\hline
Other & 21-25 & Forest (2), Rural (2), Urban (1) & Rainy (2), Windy (1), Clear (2) & Day (3), Night (2) & Moderate (4), Complex (1) \\
\hline
\end{tabular}
\caption{Scenario Distribution across Use-Cases}
\label{tab:scenario_distribution}
\end{table*}

==> tables/technical-stack.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Component} & \textbf{Model} & \textbf{Source} \\
\hline
LLM Model & Microsoft Phi-3-medium-128k-instruct &  \cite{microsof_phi3_medium:online}\\
\hline
Vision LLM Model & Phi-3-vision-128k-instruct & \cite{microsof_phi3Vision__medium:online} \\
\hline
Embedding Model & sentence-transformers/all-mpnet-base-v2 & \cite{sentence29:online} \\
\hline
% Vector DB & FAISS \\
% \hline
\end{tabular}
\caption{Source of core LLM components}
\label{tab:tech_stack}
\end{table}
